KALA: Knowledge-Augmented Language Model Adaptation

Pre-trained language models (PLMs) have achieved remarkable success on various natural language understanding tasks. Simple fine-tuning of PLMs, on the other hand, might be suboptimal for domain-specific tasks because they cannot possibly cover knowledge from all domains. While adaptive pre-training of PLMs can help them obtain domain-specific knowledge, it requires a large training cost. Moreover, adaptive pre-training can harm the PLM's performance on the downstream task by causing catastrophic forgetting of its general knowledge. To overcome such limitations of adaptive pre-training for PLM adaption, we propose a novel domain adaption framework for PLMs coined as Knowledge-Augmented Language model Adaptation (KALA), which modulates the intermediate hidden representations of PLMs with domain knowledge, consisting of entities and their relational facts. We validate the performance of our KALA on question answering and named entity recognition tasks on multiple datasets across various domains. The results show that, despite being computationally efficient, our KALA largely outperforms adaptive pre-training. Code is available at: https://github.com/Nardien/KALA/.

==> figures/casestudy.tex <==
\begin{figure}[t!]
    \begin{minipage}{0.42\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
            \begin{tabular}{lccl}
            \toprule
            \makecell[l]{Context:
                    A \BLUE{nonsense mutation} in \\
                    \BLUE{exon} 17 ( \BLUE{codon} 556 ) of the RB1 \\
                    \BLUE{gene} was found to be present \\
                    homozygously in both the \RED{retinal} \\ 
                    and the pineal tumours.
            } \\
            \midrule
            Fact: (retinal, instance of, gene) \\
            \bottomrule
            \end{tabular}
        }
    \end{minipage}
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/casestudy/vanila.pdf}
    \end{minipage}
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/casestudy/v1.pdf}
    \end{minipage}
    \vspace{-0.125in}
    \caption{\small A case study on one context of the NCBI-Disease dataset. A left table shows the context and its fact, and a right figure shows a visualization of token representations. Text in blue and red denote the seen and unseen entities, respectively.}
    \label{fig:casestudy}
    \vspace{-0.15in}
\end{figure}


==> tables/efficiency.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/memory/memory.pdf}
    \caption{\small NewsQA results of varying size of the Entity Memory (left) and the GPU Memory needed for training (right). We remove less frequent entities first when the size of entity memory decreases.}
    \vspace{-0.2in}
\end{figure}


==> tables/qa-ablation-1.tex <==
\begin{table}
	\centering
	\small
	\resizebox{0.8\columnwidth}{!}{
	\begin{tabular}{lcc}
		\toprule
		{\textbf{K-FiLM Components (\S3.2)}} & \multicolumn{2}{c}{\textbf{NewsQA}}  \\
		\textbf{BERT-base}                   & EM          & F1          \\ 
		\midrule[0.8pt]
		\textbf{None (Fine-tuning)} & {52.87} & {67.10}\\
		\textbf{+ $\bm{\Gamma}, \bm{\tilde{\Gamma}}$} \textit{(gamma only)}& {53.81} & {67.70}\\
		\textbf{+ $\mB, \tilde{\mB}$} \textit{(beta only)} & {52.92} &  {67.20}\\
		\textbf{+ $\bm{\Gamma}, \mB$} \textit{(first only)} & {53.16} & {66.97}\\
		\textbf{+ $ \bm{\tilde{\Gamma}}, \tilde{\mB}$} \textit{(second only)} & {53.61} & {67.90}\\
		\midrule[0.8pt]
		\textbf{+ $\bm{\Gamma}, \mB, \bm{\tilde{\Gamma}}, \tilde{\mB}$ (\textbf{final})} & {\textbf{54.95}} &  {\textbf{68.56}}\\
		\bottomrule
	\end{tabular}
	}
	\caption{\small Ablation study of the K-FiLM Components $\bm{\Gamma}$, $\mB$, $\bm{\tilde{\Gamma}}$, $\tilde{\mB}$ on the \RED{NewsQA} dataset with BERT-base. (3 seeds)}
	\label{table:ablationfilm}
\end{table}


==> tables/qa-ablation-2.tex <==
\begin{table}
	\centering
	\small
	\resizebox{0.8\columnwidth}{!}{
	\begin{tabular}{lcc}
		\toprule
		{\textbf{Architecture Variants (\S5.2)}} & \multicolumn{2}{c}{\textbf{NewsQA}}  \\
		\textbf{BERT-base}                   & EM          & F1          \\ 
		\midrule[0.8pt]
		\textbf{ERNIE}~\citep{ERNIE} & {53.35} &  {67.49}\\ 
		\textbf{Adapter}~\citep{HoulsbyAdapter} & {53.32} & {67.38}\\ 
		\textbf{KT-Net}~\citep{KTNet}$^\dagger$ & {53.32} & {66.78} \\ 
		\textbf{EaE}~\citep{EaE}& {53.00} & {67.40}\\ 
		\textbf{ERICA}~\citep{ERICA} & {51.99} & {66.40}\\ 
		\midrule[0.8pt]
		\textbf{KALA (ours)} & {\textbf{54.16}} & {\textbf{68.22}}\\
		\bottomrule
	\end{tabular}
	}
	\caption{\small Experimental results on knowledge integration architecture variants on the \RED{NewsQA} dataset with BERT-base.}
\end{table}


==> tables/qa-ablation-3.tex <==
\begin{table}
	\centering
	\small
	\resizebox{0.8\columnwidth}{!}{
	\begin{tabular}{lcc}
		\toprule
		{\textbf{Graph Attention (\S3.3)}} & \multicolumn{2}{c}{\textbf{NewsQA}}  \\
		\textbf{BERT-base}                   & EM          & F1          \\ 
		\midrule[0.8pt]
		\textbf{$\ve_i, \ve_j$} \textit{(only entity emb.)} & {54.35} & {68.27}\\
		\textbf{+ $\vr_{ij}$} \textit{(with relation emb.)}   & {53.76} & {67.60}\\
		\textbf{+ $\vh_{e_i}$} \textit{(with LM representation)}  & {53.49} & {67.47}\\
		\midrule[0.8pt]
		\textbf{+ $\vr_{ij}, \vh_{e_i}$ (\textbf{final})} & {\textbf{54.95}} &  {\textbf{68.56}}\\
		\bottomrule
	\end{tabular}
	}
	\caption{\small Ablation study of the Graph Attention Components for consisting $\vh^*$ on the \RED{NewsQA} dataset with BERT-base. (3 seeds)}
	\label{table:ablationgraph}
\end{table}


==> tables/qa-ablation-all.tex <==
\begin{figure*}[!t]
    \begin{minipage}{0.32\linewidth}
        \centering
        \resizebox{1.0\textwidth}{!}{
        \renewcommand{\tabcolsep}{1.0mm}
        \begin{tabular}{lcc}
		\toprule
		{\textbf{KFM Components (\S3.2)}    } & \multicolumn{2}{c}{\textbf{NewsQA}}  \\
		\textbf{BERT-base}                   & EM          & F1          \\ 
		\midrule[0.8pt]
		\textbf{None (Fine-tuning)} & {52.87} & {67.10}\\
		\textbf{+ $\bm{\Gamma}, \bm{\tilde{\Gamma}}$} \textit{(gamma only)}& {53.81} & {67.70}\\
		\textbf{+ $\mB, \tilde{\mB}$} \textit{(beta only)} & {52.92} &  {67.20}\\
		\textbf{+ $\bm{\Gamma}, \mB$} \textit{(first only)} & {53.16} & {66.97}\\
		\textbf{+ $ \bm{\tilde{\Gamma}}, \tilde{\mB}$} \textit{(second only)} & {53.61} & {67.90}\\
		\midrule[0.8pt]
		\textbf{+ $\bm{\Gamma}, \mB, \bm{\tilde{\Gamma}}, \tilde{\mB}$ (\textbf{final})} & {\textbf{54.95}} &  {\textbf{68.56}}\\
		\bottomrule
    	\end{tabular}
    	}
    	\vspace{0.04in}
    	\captionof{table}{\small Ablation study of the K-FiLM Components $\bm{\Gamma}$, $\mB$, $\bm{\tilde{\Gamma}}$, $\tilde{\mB}$. (3 seeds)}
    	\label{table:ablationfilm}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \vspace{0.26in}
        \centering
        \resizebox{1\textwidth}{!}{
        \renewcommand{\tabcolsep}{1.0mm}
        \begin{tabular}{lcc}
		\toprule
		{\textbf{Graph Attention (\S3.3)}} & \multicolumn{2}{c}{\textbf{NewsQA}}  \\
		\textbf{BERT-base}                   & EM          & F1          \\ 
		\midrule[0.8pt]
		\textbf{$\ve_i, \ve_j$} \textit{(only entity emb.)} & {54.35} & {68.27}\\
		\textbf{+ $\vr_{ij}$} \textit{(with relation emb.)}   & {53.76} & {67.60}\\
		\textbf{+ $\vh_{e_i}$} \textit{(with LM representation)}  & {53.49} & {67.47}\\
		\midrule[0.8pt]
		\textbf{+ $\vr_{ij}, \vh_{e_i}$ (\textbf{final})} & {\textbf{54.95}} &  {\textbf{68.56}}\\
		\bottomrule
    	\end{tabular}
    	}
    	\captionof{table}{\small Ablation study of the Graph Attention Components for consisting $\vh^*$. (3 seeds)}
	\label{table:ablationgraph}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \resizebox{1\textwidth}{!}{
        \renewcommand{\tabcolsep}{1.0mm}
        \begin{tabular}{lcc}
		\toprule
		{\textbf{Architecture Variants (\S5.2)}} & \multicolumn{2}{c}{\textbf{NewsQA}}  \\
		\textbf{BERT-base}                   & EM          & F1          \\ 
		\midrule[0.8pt]
		\textbf{ERNIE}~\citep{ERNIE} & {53.35} &  {67.49}\\
		\textbf{Adapter}~\citep{HoulsbyAdapter} & {53.32} & {67.38}\\
		\textbf{KT-Net}~\citep{KTNet} & {53.15} & {67.01} \\
		\textbf{EaE}~\citep{EaE}& {53.00} & {67.40}\\
		\textbf{ERICA}~\citep{ERICA} & {51.99} & {66.40}\\
		\midrule[0.8pt]
		\textbf{KALA (ours)} & {\textbf{54.16}} & {\textbf{68.22}}\\
		\bottomrule
    	\end{tabular}
    	}
    	\captionof{table}{\small Experimental results on knowledge integration architecture variants.}
	\label{table:variants}
	\end{minipage}
    \vspace{-0.1in}
\end{figure*}

==> tables/qa-exp.tex <==
\begin{table*}
	\centering
	\small
	\resizebox{0.9\textwidth}{!}{
	\begin{tabular}{lccc}
		\toprule
		{\textbf{Method}} & \textbf{NewsQA} & {\textbf{Relation}} & {\textbf{Medication}} \\
		\midrule[0.8pt]
		\multicolumn{4}{c}{\textbf{BERT-base} (EM | F1) } \\
		\midrule[0.8pt]
		\textbf{Fine-Tuning} & {52.87 $\pm$ 0.91 | 67.10 $\pm$ 0.13} & {54.76 $\pm$ 0.93 | 62.27 $\pm$ 0.61} & {\textbf{12.70} $\pm$ 0.20 | 43.42 $\pm$ 1.04} \\
		\textbf{+} \textit{more params} & {53.02 $\pm$ 1.09 | 67.35 $\pm$ 0.62} & {53.82 $\pm$ 1.94 | 61.90 $\pm$ 2.08} & {12.60 $\pm$ 0.27 | 42.46 $\pm$ 1.18}  \\
		\textbf{TAPT} & {53.17 $\pm$ 1.62 | 66.69 $\pm$ 1.47} & {53.48 $\pm$ 3.24 | 60.45 $\pm$ 3.87} & {12.57 $\pm$ 0.63 | 43.35 $\pm$ 1.32}  \\
		\textbf{+ RecAdam} & {53.36 $\pm$ 0.67 | 66.99 $\pm$ 1.25} & {56.34 $\pm$ 1.04 | 64.22 $\pm$ 0.91} & {12.70 $\pm$ 0.46 | 43.80 $\pm$ 1.32} \\
		\midrule[0.5pt]
		\textbf{KALA} \textit{(point-wise)} & {53.71 $\pm$ 0.93 | 67.67 $\pm$ 0.69} & {52.63 $\pm$ 2.76 | 63.07 $\pm$ 2.34} & {12.07 $\pm$ 0.55 | 43.22 $\pm$ 0.64} \\
		\textbf{KALA} \textit{(dense)} & {53.86 $\pm$ 0.91 | 68.17 $\pm$ 0.84} & {55.65 $\pm$ 0.94 | 63.05 $\pm$ 0.46} & {12.26 $\pm$ 0.75 | 43.19 $\pm$ 1.36} \\
		\textbf{KALA} \textit{(dense, sup)} & {52.97 $\pm$ 0.68 | 67.31 $\pm$ 0.46} & {53.40 $\pm$ 0.18 | 61.27 $\pm$ 1.24} & {11.90 $\pm$ 0.36 | 41.38 $\pm$ 0.49} \\
		\textbf{KALA} \textit{(relational)} & {\textbf{54.95} $\pm$ 0.08 | \textbf{68.56} $\pm$ 0.29} & {\textbf{57.07} $\pm$ 1.27 | \textbf{65.29} $\pm$ 1.26} & {12.41 $\pm$ 0.41 | \textbf{44.54} $\pm$ 0.45}  \\
		\bottomrule
	\end{tabular}
	}
	\caption{\small Experimental results of the extractive QA task on four different datasets with the BERT-base. The reported results are means and standard deviations over three different runs. The numbers in bold fonts denote the best score. (ver: 20211008)}
	\label{qa-exp}
\end{table*}



==> tables/qa-generative.tex <==
\begin{table}
    \vspace{0.075in}
	\centering
	\small
	\resizebox{0.75\columnwidth}{!}{
	\renewcommand{\arraystretch}{1.05}
    \renewcommand{\tabcolsep}{5.0mm}
    \begin{tabular}{lcc}
    	\toprule
    	                                   & \multicolumn{2}{c}{\textbf{NewsQA}}  \\
    	\textbf{T5-small}                   & EM          & F1          \\ 
    	\midrule[0.8pt]
    	\textbf{Fine-tuning} & {48.96} &  {64.24}\\
    	\textbf{TAPT}        & {48.66} &  {64.30} \\
    	+ \textbf{RecAdam}   & {48.37} &  {63.41} \\
    	\midrule[0.8pt]
    	\textbf{KALA (ours)} & {\textbf{51.78}} & {\textbf{66.88}}\\ 
    	\bottomrule
    \end{tabular}
	}
	\vspace{-0.05in}
	\caption{\small Experimental results on generative question answering with T5-small as a PLM and NewsQA as a dataset.}
	\label{table:generative-qa}
	 \vspace{-0.15in}
\end{table}

